On Finding Gray Pixels

We propose a novel grayness index for finding gray pixels and demonstrate its effectiveness and efficiency in illumination estimation. The grayness index, GI in short, is derived using the Dichromatic Reflection Model and is learning-free. GI allows to estimate one or multiple illumination sources in color-biased images. On standard single-illumination and multiple-illumination estimation benchmarks, GI outperforms state-of-the-art statistical methods and many recent deep methods. GI is simple and fast, written in a few dozen lines of code, processing a 1080p image in ~0.4 seconds with a non-optimized Matlab code.

==> Makefile <==
# original Makefile by Pasi "okun" Valminen, 2004
# edited by Pekka "PQ" Paalanen, 2004 - 2007
# version 4.1.2007

## Modify these to your needs.

SHELL=/bin/bash

# document target basename
TARGET   := cvpr2018

# Autogenerated source files, like eps-figures created with
# gnuplot scripts. Target 'distclean' will delete files listed here.
AUTOTGT  := 
            

## The following should be ok as is.

# document source files
SRC      := $(wildcard *.tex) $(wildcard *.bib) $(AUTOTGT)

# programs
GS       := gs
TEXI2PDF := texi2pdf
GNUPLOT  := gnuplot
EPS2PDF  := epstopdf

GSPDF_OPTS := -sDEVICE=pdfwrite -dPDFSETTINGS=/printer \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true \
              -dEmbedAllFonts=true

# The GS options are from http://www.ctan.org/tex-archive/macros/latex/
#   contrib/IEEEtran/testflow/testflow_doc.txt

# Texi2pdf runs bibtex automatically and pdflatex as many times as needed.

all: $(TARGET).pdf

clean:
	rm -f *.{aux,bbl,blg,tmp,dvi,toc,log,out,idx,ilg,ind,brf,spl} *~

distclean: clean
	rm -f $(AUTOTGT) $(AUTOTGT:.pdf=.eps) $(TARGET).pdf

view: $(TARGET).pdf
	xpdf -remote view-$(abspath $(TARGET).pdf) $(TARGET).pdf &

%.pdf: %.tex $(SRC)
	$(TEXI2PDF) $<

%.eps: %.gp
	$(GNUPLOT) $<

%.pdf: %.eps
	epspdf $<
#	$(EPS2PDF) --nogs $< | $(GS) -q $(GSPDF_OPTS) \
#	  -dAutoRotatePages=/None -sOutputFile=$@ - -c quit

.SUFFIXES:
.PRECIOUS: %.dvi %.pdf
.DELETE_ON_ERROR: %.dvi %.pdf
.PHONY: all clean distclean view

